Matrix model approximations of fuzzy scalar field theories and their phase diagrams

We present an analysis of two different approximations to the scalar field theory on the fuzzy sphere, a nonperturbative and a perturbative one, which are both multitrace matrix models. We show that the former reproduces a phase diagram with correct features in a qualitative agreement with the previous numerical studies and that the latter gives a phase diagram with features not expected in the phase diagram of the field theory.

==> 3_sym_old.tex <==
In the light of the lessons learnt in the previous section, we proceed to the calculation of the phase diagram of the theory given by the action (\ref{}). We will first deal with the one-cut to two-cut phase transition, which is symmetric and thus we can set the odd moments to zero, simplifying the calculations considerably. Then, we will consider the symmetric to asymmetric phase transition and finally we will locate the triple point of the model and compare it with the triple point of the previous model (\ref{}).

Our analysis will results on two surprising conclusions. The triple point will be shifted further away from the numerical value (\ref{}), having an opposite effect to the expected one. Moreover, the perturbative series for the one-cut to two-cut phase transition line will change its behaviour rather drastically.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{One-cut to two cut phase transition}

With the odd moments set to zero, the effective action for the model up to fourth order in kinetic term reads
\be S_{eff}=\half\lr{\ep A_1 c_2+\ep^2 A_2 c_2^2+\ep^3 A_3 c_2^3+\ep^4 A_4 c_2^4}+C \ep^4 \lr{c_4-2c_2^2}^2\ .\ee
We could in principle include terms of higher order in $\ep$ from the $F(c_2)$ part, but we will not do that at the moment. The corresponding saddle point equation for the eigenvalue distribution is given by
\be \lr{\ep A_1 +\ep^2 2 A_2 c_2+\ep^3 A_3 3 c_2^2+\ep^4 A_4 4 c_2^3}x+C \ep^4 2\lr{c_4-2c_2^2}(4x^3-8c_2 x)+r x+4gx^3=\int dx'\frac{\rho(x')}{x-x'}\ ,\ee
which can be written in the terms of effective mass and effective coupling
\begin{align}
r_{eff}x+4g_{eff}x^3=&\int dx'\frac{\rho(x')}{x-x'}\\
&r_{eff}=r+\lr{\ep A_1 +\ep^2 2 A_2 c_2+\ep^3 A_3 3 c_2^2+\ep^4 A_4 4 c_2^3}\no&\ \ \ \ \ \ -16C \ep^4 2\lr{c_4-2c_2^2}c_2\\
&g_{eff}=g+C \ep^4 2\lr{c_4-2c_2^2}
\end{align}
The phase transition of this model is then given by the equation
\be r_{eff}=-4\sqrt{g_{eff}}\ee
Having an expression for the moments $c_2,c_4$ in terms of parameters $r,g$, we can find the solution of this equation as a perturbatve series in $\ep$. The result reads
\be r(g)=-4\sqrt{g}-A_1-\frac{2A_2}{\sqrt g}-\frac{3A_3}{g}-\frac{4A_4+9C}{g^{3/2}}\ .\ee
We can clearly identify the $9C/g^{3/2}$ correction to the transition line (\ref{}). As mentioned in the previous section, this formula as it stands is of little use, since the series it comes from is not well behaved for small values of $g$ and needs some further treatment. To do that, we concentrate on the case of the fuzzy sphere, where the numerical values of the coeficients are known. We obtain
\be r(g)=-4 \sqrt g - \half +\frac{1}{12\sqrt g}+\frac{7}{5760 g^{3/2}}\ .\ee
We can see a change of sign in the last term.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Symmetric to asymmetric phase transition}

The full action (\ref{}) with the odd terms included is rather complicated, but it is still straightforward to write down the saddle point equation
\be a_{eff}+r_{eff}x+3 h_{eff}x^2+4g_{eff}x^3=\int dx'\frac{\rho(x')}{x-x'} \ee
where we have placed the cumbersome expressions for the coefficients to the appendix. This corresponds again to a potential with two minima that have unequal depths. For certain values of parameters, one well an be deep enough to house all the eigenvalues and thus make the asymmetric one cut solution possible. In terms of the effective parameters, this happens when (\ref{})
\be \ .\ee
We again look for the solution of this equation as a power series in $\ep$, obtaining
\begin{align}
r(g)=&-2 \sqrt{15} \sqrt{g}+ \ep \frac{4 A_1}{5}+\ep^2 \frac{135 A_1^2 + 848 A_2}{
 1500 \sqrt{15} \sqrt{g}}+\ep^3\frac{
 2025 A_1^3 + 10170 A_1 A_2 + 11236 A_3 + 11556 B}{562500 g}+\no&+\ep^4\frac{\begin{array}{l}
 5740875 A_1^4 + 32464800 A_1^2 A_2 + 19805040 A_2^2 +\\ 29707560 A_1 A_3 + 
  19056256 A_4 + 35069760 A_1 B + 85332800 C\end{array}}{
 2025000000 \sqrt{15} g^{3/2}}
\end{align}
with an extra fourth order terms as expected. For the fuzzy sphere, this yields
\be r(g)= - 2 \sqrt{15} \sqrt{g}+\frac{2}{5}- \frac{19}{18000 \sqrt{15} \sqrt{g}}+ \frac{29}{
 1125000 g} - \frac{64359383}{4374000000000 \sqrt{15} g^{3/2}} \ .\label{3kuk}\ee
We see that in this case the series is still alternating and thus we do not run into the same problems as for the one-cut to two-cut transition. This means we can safely use the approximation techniques of section \ref{sec2} to continue series (\ref{3kuk}) to small values of $g$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The triple point}

==> 45_renorm.tex <==
uff

==> 4_asym_old.tex <==
As mentioned in the section \ref{sec2}, due to quantum fluctuations the pure matrix theory with negative coupling constant $g<0$ does not have stable eigenvalue configurations for any value of $r$. However in the same section we have seen that the kinetic term effective action introduces terms, which change the value of $g$. Namely, up to fourth order in the kinetic term, we have obtained the effective coupling
\be g_{eff}=g+2 F \lr{c_{40}-2 c_{20}^2}\ .\ee
And finally, for the fuzzy sphere cases we have obtained a negative coefficient $F<0$. This means, that for there is a possibility that a distribution with $c_{40}-2c_{20}^2$ negative enough can overcome the negativity of the original coupling constant and we can have a stable eigenvalue distribution even for $g<0$.

Quantity $c_{40}-2c_{20}^2$ describes how far apart the eigenvalues are. It vanishes for the semicircle distribution and is negative for distributions, that have more eigenvalues away from the mean value than the semicircle. This means that we expect the two cut solution to survive the case of negative coupling and sooner or later spread enough to make the effective coupling positive. However, it is not clear at the moment whether the one cut distributions will have $c_{40}-2c_{20}^2$ negative enough to stabilize.

After this short introduction, we can proceed with the computation of the region of existence of the three possible cases of the eigenvalue distributions.

\paragraph{Double cut distribution}

We start with computationally the simplest case. This solution to the equation (\ref{}) exists, if
\be g_{eff}>0 \ , \ r_{eff}<-4\sqrt{g_eff}\ .\ee
In the case of $g>0$ these two conditions became
\be r(g)=-4\sqrt{g}-\half+ \ ,\ee
formula we dealt with extensively in the section (\ref{sec3}). For $g<0$, we again look for the lines $r(g)$, where the conditions become equalities. To do this, we simply put the expression equal to zero, solve for $r$ and keep in mind that we have right to consider only the terms up to order $\ep^4$. Using the explicit formulas for the second and fourth moments, we obtain for the first of the conditions
\begin{subequations}
\be r(g)=\ \frac{1}{\ep^2}2\sqrt 2\sqrt{-\frac{g^3}{F}}+\ep^2\sqrt 2 \sqrt{\frac{F}{g}},\ee
while the second
\be r(g)=\ -4\sqrt.\ee
Moreover, we require that the distribution is always positive and the two parameters that describe it, $D$ and $\delta$ are real and positive, yielding
\be
r(g)= 
\ee
and
\be r(g)= \ee
\end{subequations}
respectively. These four conditions are show in the figure.

As before, these are divergent expression in the limit of $g\to0$ and we need to use some method to control the behavior in the proximity of the origin of the phase diagram. The first two equations expressions also diverge in the limit of pure matrix model $\ep\to0$, which might be bothering. However this is expected, as the two equations represent effects that are not present in the pure matrix model and this removes them completely from the diagram in this limit.

\paragraph{Symmetric single cut distribution}

For the symmetric single cut distribution to exists (to be non-negative), we have the complementary condition
\be g_{eff}>0 \ , \ r_{eff}>-4\sqrt{g_eff}\ ,\ee
however with the corresponding moments of the different case of the distribution. With the condition of positive and real $\delta$, we get the following boundaries of the region of validity of the symmetric single cut assumption
\begin{align}
r(g)&= \ ,\\
r(g)&= \ ,\\
r(g)&= \ .
\end{align}

\paragraph{Asymmetric single cut distribution}

